Characterization and Learning of Causal Graphs with Small Conditioning Sets

Constraint-based causal discovery algorithms learn part of the causal graph structure by systematically testing conditional independences observed in the data. These algorithms, such as the PC algorithm and its variants, rely on graphical characterizations of the so-called equivalence class of causal graphs proposed by Pearl. However, constraint-based causal discovery algorithms struggle when data is limited since conditional independence tests quickly lose their statistical power, especially when the conditioning set is large. To address this, we propose using conditional independence tests where the size of the conditioning set is upper bounded by some integer $k$ for robust causal discovery. The existing graphical characterizations of the equivalence classes of causal graphs are not applicable when we cannot leverage all the conditional independence statements. We first define the notion of $k$-Markov equivalence: Two causal graphs are $k$-Markov equivalent if they entail the same conditional independence constraints where the conditioning set size is upper bounded by $k$. We propose a novel representation that allows us to graphically characterize $k$-Markov equivalence between two causal graphs. We propose a sound constraint-based algorithm called the $k$-PC algorithm for learning this equivalence class. Finally, we conduct synthetic, and semi-synthetic experiments to demonstrate that the $k$-PC algorithm enables more robust causal discovery in the small sample regime compared to the baseline algorithms.

==> exp-synthetic-table.tex <==

\begin{table}[t!]
\caption{Performance comparison between  \kPC for $k=1$ and PC on average over randomly generated linear Gaussian SCMs on causal graph $D_1$ in Figure \ref{fig:warmup}. $N:$ Number of samples. \kPC leads to improved skeleton and arrowhead mark discovery in the small sample regime, with a minor tradeoff at tail mark discovery.}
\label{fig:my_label}
\vskip 0.15in    
\footnotesize
\centering
    \hspace{-2.5em}
    \begin{subtable}[h]{.2\textwidth}
    \centering
    \begin{tabular}{ l | c c c}
    \backslashbox{}{$N\!\!$}& $10^2$ & $10^3$ &$10^4$\\
    \hline 
     \kPC & \textbf{0.84} & 0.88 & 0.89\\ 
     PC & 0.80 & \textbf{0.93} & \textbf{0.99}
    \end{tabular}
    \caption{Skeleton F1 Score}
    \end{subtable}
    \hspace{4em}
    \begin{subtable}[h]{.2\textwidth}
    \centering
    \begin{tabular}{ l | c c c}
        \backslashbox{}{$N\!\!$}&  $10^2$ & $10^3$ &$10^4$\\
    \hline 
     \kPC & \textbf{0.54} & \textbf{0.71} & 0.75\\ 
     PC & 0.04 & 0.54 & \textbf{0.9}
    \end{tabular}
    \caption{Arrowhead F1 Score}
    \end{subtable}
    \hspace{4em}
    \begin{subtable}[h]{.2\textwidth}
    \centering
    \begin{tabular}{ l | c c c}
        \backslashbox{}{$N\!\!$}& $10^2$ & $10^3$ &$10^4$\\
    \hline 
     \kPC & 0.55 & 0.71 & 0.75\\ 
     PC & \textbf{0.58} & \textbf{0.81} & \textbf{0.96}
    \end{tabular}
    \caption{Tail F1 Score}
    \end{subtable}
    \vspace{-2em}
\end{table}


==> preamble.tex <==
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{mathtools}

\usepackage{color}

\usepackage{diagbox}



\newcommand{\indep }{\perp\!\!\!\perp}
\newcommand{\ci}[3]{#1 \indep #2 \left\vert #3\right.}
\newcommand{\nci}[3]{#1 \not\!\perp\!\!\!\perp #2 \left\vert #3\right.}
\newcommand{\nmi}[2]{#1 \not\!\perp\!\!\!\perp #2}

\newcommand{\red}[1]{{\color{red} #1}}

\newcommand{\bl}[1]{{\color{blue} #1}}

\DeclareSymbolFont{symbolsC}{U}{txsyc}{m}{n}
\DeclareMathSymbol{\notniFromTxfonts}{\mathrel}{symbolsC}{61}

\newcommand{\C}[1]{\mathcal{C}_k(#1)}
\newcommand{\E}[1]{\varepsilon_k(#1)}
\newcommand{\R}[1]{$\mathcal{R}#1$}
\newcommand{\FCIp}[1]{\text{FCI+}(#1)}
\newcommand{\FCI}[1]{\text{FCI}(#1)}
\newcommand{\PAG}[1]{\text{PAG}(#1)}
\newcommand{\degree}[1]{degree-$#1$}

\newcommand{\srightarrow}{*\!\!\rightarrow}
\newcommand{\sleftarrow}{\leftarrow\!\!*}
\newcommand{\starstar}{*\!\!\mbox{---}\!\!*}

\newcommand{\scircle}{*\!\!$\mbox{---}$o}
\newcommand{\circlecircle}{o\mbox{---}o}
\newcommand{\circlestar}{o\mbox{---}\!*}
\newcommand{\starcircle}{*\!\mbox{---}o}
\newcommand{\tailstar}{\mbox{---}*}

\newcommand{\crightarrow}{o\!\!\rightarrow}
\newcommand{\cleftarrow}{\leftarrow\!\!o}
\newcommand{\cleftrightarrow}{o$\mbox{---}$o }
\newcommand{\kmarkov}{$k$-Markov }
\newcommand{\kclosure}{$k$-closure }
\newcommand{\kclosures}{$k$-closures}
\newcommand{\kcovered}{$k$-covered }
\newcommand{\kessential}{$k$-essential }
\newcommand{\dkci}{degree-$k$ d-separation }
\newcommand{\kPC}{$k$-PC }

\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes,backgrounds}
\tikzset{
	circ/.style = {circle, draw, inner sep=0.04cm,node contents={}}
}
\usetikzlibrary{positioning}
\usepackage{graphicx}
\usepackage{wrapfig}





\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{booktabs} %

\usepackage{hyperref}


\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

\usepackage{algorithmic}
\usepackage{algorithm}

\usepackage[capitalize,noabbrev]{cleveref}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\usepackage[textsize=tiny]{todonotes}
